TLDR: Text Based Last-layer Retraining for Debiasing Image Classifiers

An image classifier may depend on incidental features stemming from a strong correlation between the feature and the classification target in the training dataset. Recently, Last Layer Retraining (LLR) with group-balanced datasets is shown to be efficient in mitigating the spurious correlation of classifiers. However, the acquisition of image-based group-balanced datasets is costly, which hinders the general applicability of the LLR method. In this work, we propose to perform LLR based on text datasets built with large language models to debias a general image classifier. To that end, we demonstrate that text can generally be a proxy for its corresponding image beyond the image-text joint embedding space, which is achieved with a linear projector that ensures orthogonality between its weight and the modality gap of the joint embedding space. In addition, we propose a systematic validation procedure that checks whether the generated words are compatible with the embedding space of CLIP and the image classifier, which is shown to be effective for improving debiasing performance. We dub these procedures as TLDR (Text-based Last layer retraining for Debiasing image classifieRs) and show our method achieves the performance that is competitive with the LLR methods that require group-balanced image dataset for retraining. Furthermore, TLDR outperforms other baselines that involve training the last layer without any group annotated dataset. Codes: https://github.com/beotborry/TLDR

==> Table/spuco_animal_table.tex <==
\resizebox{\columnwidth}{!}{%

\begin{tabular}{c c c cc}

\multirow{2}{*}{\textbf{Method}} & \textbf{Group Info} & \textbf{Use Given Model} &\multicolumn{2}{c}{\textbf{SpuCoAnimals}}
\\

\cline{4-5}
\\[-3mm]
& Train / Val & &
Worst(\%) & Mean(\%)
\\[1mm]\hline\\[-3mm]

ERM &
\ding{55} / \ding{55} & -
&$6.3_{\pm 1.6}$ & $81.3_{\pm 0.9}$
\\

\DFRVAL &
\ding{55} / \checkmark\checkmark & \checkmark
&$38.3_{\pm9.3}$ & $60.0_{\pm3.8}$
\\

AFR &
\ding{55} / \checkmark & \ding{55}
&$15.6_{\pm6.0}$ & $61.1_{\pm1.8}$
\\

AFR (with given ERM) &
\ding{55} / \checkmark & \checkmark
&$22.3_{\pm3.4}$ & $53.8_{\pm7.7}$
\\

SELF &
\ding{55} / \checkmark & \ding{55}
\\

SELF (with given ERM) &
\ding{55} / \checkmark & \checkmark
\\


CLIPREC &
\ding{55} / \checkmark & \checkmark
% &$38.9_{\pm 3.1}$ & $61.3_{\pm 0.7}$
\end{tabular}
}

==> Table/t_test_filtering.tex <==
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{c c cc c cc c cc c cc c cc}

\toprule
\multirow{2}{*}{\textbf{Used Filter}} & \multicolumn{2}{c}{\textbf{Waterbirds}} & \multicolumn{2}{c}{\textbf{CelebA}} & \multicolumn{2}{c}{\textbf{SpuCoAnimals}}
\\

\cline{2-7}
\\[-3mm]
& Worst(\%) & Mean(\%) & 
Worst(\%) & Mean(\%) &
Worst(\%) & Mean(\%) &
\\[1mm]
\midrule
Full (Tab. \ref{tab:ablation_filter})
& $92.1_{\pm0.3}$ & $95.2_{\pm0.8}$
& $85.4_{\pm1.2}$ & $89.0_{\pm0.9}$
& $36.2_{\pm1.7}$ & $55.8_{\pm2.9}$
\\
Replace $\mathcal{T}^a$ semantic filter with t-test
& $92.1_{\pm0.5}$ & $95.5_{\pm0.4}$
& $84.8_{\pm1.1}$ & $89.2_{\pm0.9}$
& $33.2_{\pm6.7}$ & $58.6_{\pm2.4}$
\\

Full + t-test 
& $92.1_{\pm0.5}$ & $95.4_{\pm0.5}$
& $85.4_{\pm1.2}$ & $89.0_{\pm0.9}$
& $35.8_{\pm5.3}$ & $55.4_{\pm2.6}$
\\
\bottomrule
\end{tabular}
}

==> Table/urban_cars_table.tex <==
\begin{tabular}{c c cc c cc c cc c cc}

\multirow{2}{*}{\textbf{Method}} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{UrbanCars}}
\\

\cline{3-4}
\\[-3mm]
& Train / Val & 
Worst(\%) & Mean(\%)
\\[1mm]\hline\\[-3mm]

ERM (Ours) &
\ding{55} / \ding{55}
\\

LLE &
\ding{55} / \checkmark\checkmark
\\

LLE(Ours) &
\ding{55} / \checkmark\checkmark
\\

LLE + CLIPREC &
\ding{55} / \ding{55}

\\[1mm]\hline

\end{tabular}

==> Table/waterbirds_celeba_table_old.tex <==
\begin{tabular}{c c cc c cc c cc c cc}

\multirow{2}{*}{\textbf{Method}} & \textbf{Group Info} & \multicolumn{2}{c}{\textbf{Waterbirds}} && \multicolumn{2}{c}{\textbf{CelebA}}
\\

\cline{3-4}
\cline{6-7}
\\[-3mm]
& Train / Val & 
Worst(\%) & Mean(\%)
&& Worst(\%) & Mean(\%)
\\[1mm]\hline\\[-3mm]

JTT & 
\ding{55} / \checkmark &
86.7 & 93.3 
&& 81.1 & 88.0
\\

CnC & 
\ding{55} / \checkmark 
& $88.5_{\pm0.3}$ & $90.9_{\pm0.1}$
&& $88.8_{\pm0.9}$ & $89.9_{\pm0.5}$
\\

SUBG & 
\checkmark / \checkmark 
&
$89.1_{\pm1.1}$ & -
&& $85.6_{\pm2.3}$ & -
\\

SSA & 
\ding{55} / \checkmark\checkmark
& $89.0_{\pm0.6}$ & $92.2_{\pm0.9}$
&& $\mathbf{89.8}_{\pm1.3}$ & $92.8_{\pm0.1}$
\\

Group DRO & 
\checkmark / \checkmark 
&
91.4 & 93.5 
&& 88.9 & 92.9
\\

\hline\\[-3mm]

ERM (from DFR) & 
\ding{55} / \ding{55} 
& $74.9_{\pm2.4}$ & $98.1_{\pm0.1}$ 
&& $46.9_{\pm2.8}$ & $95.3_{\pm0}$ 
\\

\DFRVAL & 
\ding{55} / \checkmark\checkmark
& $\mathbf{92.9}_{\pm0.2}$ & $94.2_{\pm0.4}$
&& $88.3_{\pm1.1}$ & $91.3_{\pm0.3}$
\\


AFR &
\ding{55} / \checkmark
& $\mathbf{90.4}_{\pm1.1}$ & $94.2_{\pm1.2}$
&& $\mathbf{82.0}_{\pm0.5}$ & $91.3_{\pm0.3}$
\\

SELF &
\ding{55} / \checkmark
& $\mathbf{93.0}_{\pm0.3}$ & $94.5_{\pm0.6} $
&& $\mathbf{83.9}_{\pm0.9}$ & $91.4_{\pm0.4} $
\\
[1mm]\hline

ERM (Ours) &
\ding{55} / \ding{55}
& 72.2 & 98.1
&& 47.6 & 95.1
\\

\DFRVAL (Ours) &
\ding{55} / \checkmark\checkmark
& ${92.8}$ & $95.0$
&& $86.4$ & $91.4$
\\

DISPEL(Ours) &
\ding{55} / \checkmark\checkmark
& $\mathbf{92.8}_{\pm0.5}$ & $95.0_{\pm0.7}$
&& $\mathbf{84.3}_{\pm2.4}$ & $92.2_{\pm0.4}$
\\[1mm]\hline

AFR (Ours) &
\ding{55} / \checkmark
& $87.6$ & $92.1$
&& $81.8$ & $91.0$
\\

SELF (Ours) &
\ding{55} / \checkmark
& $91.15_{\pm1.1}$ & $94.84_{\pm0.8}$
&& $77.5_{\pm4.9}$ & $92.65_{\pm0.7}$
\\[1mm]\hline

CLIPREC (Gap Reg 1) &
\ding{55} / \checkmark
&$90.0_{\pm2.3}$ & $93.4_{\pm1.5}$
&&$82.1_{\pm1.5}$ & $87.8_{\pm2.4}$
\rdelim\}{9}{0mm}[Image Val Set, Proj Optim]
\\

CLIPREC (Gap Reg 10) &
\ding{55} / \checkmark
& $91.5_{\pm0.7}$& $94.3_{\pm0.7}$
&& $82.9_{\pm2.8}$& $88.9_{\pm1.7}$
\\

CLIPREC (Gap Reg 100) &
\ding{55} / \checkmark
&$91.7_{\pm1.1}$ & $94.4_{\pm0.6}$
&& $84.3_{\pm0.8}$& $89.3_{\pm1.2}$
\\

CLIPREC (Gap Reg 1000) &
\ding{55} / \checkmark
& $\mathbf{92.0}_{\pm0.8}$& $94.7_{\pm0.6}$
&&$83.4_{\pm2.1}$ & $89.6_{\pm0.7}$
\\
CLIPREC (Add Gap 0) &
\ding{55} / \checkmark
& $87.4_{\pm3.2}$ & $92.0_{\pm1.9}$
&& $81.5_{\pm1.5}$ &   $90.8_{\pm0.2}$
\\

CLIPREC (Add Gap 1) &
\ding{55} / \checkmark
& $89.8_{\pm1.2}$& $96.5_{\pm1.2}$
&& $80.1_{\pm4.9}$& $88.6_{\pm3.6}$

\\
CLIPREC (Add Gap 10) &
\ding{55} / \checkmark
& $90.1_{\pm1.5}$& $96.7_{\pm0.8}$
&& $83.4_{\pm2.8}$& $89.2_{\pm1.6}$

\\
CLIPREC (Add Gap 100) &
\ding{55} / \checkmark
& $89.4_{\pm3.4}$& $97.2_{\pm0.4}$
&& $83.1_{\pm2.1}$& $89.8_{\pm0.9}$

\\
CLIPREC (Add Gap 1000) &
\ding{55} / \checkmark
&$90.3_{\pm1.2}$ & $97.3_{\pm0.3}$
&&$83.2_{\pm1.7}$ & $89.9_{\pm1.0}$
\\[1mm]\hline


% Analytic
CLIPREC (Gap Reg 1) &
\ding{55} / \checkmark
& $91.1_{\pm1.2}$& $92.5_{\pm0.8}$
&& $73.6_{\pm6.6}$& $92.7_{\pm1.4}$
\rdelim\}{8}{0mm}[Image Val Set, Proj Analytic]
\\
CLIPREC (Gap Reg 10) &
\ding{55} / \checkmark
&$92.0_{\pm0.9}$ & $93.6_{\pm 1.0}$
&&$84.2_{\pm2.5}$ & $89.0_{\pm1.3}$
\\

CLIPREC (Gap Reg 100) &
\ding{55} / \checkmark
&$91.8_{\pm0.6}$ & $93.7_{\pm0.9}$
&&$84.1_{\pm1.4}$ & $89.2_{\pm0.8}$
\\

CLIPREC (Gap Reg 1000) &
\ding{55} / \checkmark
&$91.6_{\pm0.6}$ & $94.4_{\pm0.5}$
&& $84.2_{\pm1.5}$& $89.2_{\pm1.3}$
\\


CLIPREC No ES (Gap Reg 1) &
\ding{55} / \checkmark
&$90.5_{\pm1.4}$ & $92.2_{\pm1.4}$
&&$56.3_{\pm19.2}$ & $94.0_{\pm1.8}$
\\
CLIPREC No ES (Gap Reg 10) &
\ding{55} / \checkmark
& $91.2_{\pm0.5}$& $93.9_{\pm0.7}$
&&$83.0_{\pm3.0}$ & $88.7_{\pm1.7}$
\\

CLIPREC No ES (Gap Reg 100) &
\ding{55} / \checkmark
&$91.4_{\pm1.0}$ & $93.1_{\pm0.7}$
&&$83.4_{\pm1.4}$ & $88.9_{\pm1.4}$
\\

CLIPREC No ES (Gap Reg 1000) &
\ding{55} / \checkmark
&$91.8_{\pm0.5}$ & $94.5_{\pm0.7}$
&&$83.1_{\pm1.7}$ & $88.4_{\pm1.8}$
\\
\\[1mm]\hline

% Analytic No Train Aug
CLIPREC (Gap Reg 1) &
\ding{55} / \checkmark
&$91.0_{\pm0.7}$& $91.9_{\pm0.6}$
&& - & - 
\rdelim\}{8}{0mm}[Proj Analytic, No train aug]

\\
CLIPREC (Gap Reg 10) &
\ding{55} / \checkmark
& $92.0_{\pm0.5}$& $93.4_{\pm0.8}$
&& - & - 
\\

CLIPREC (Gap Reg 100) &
\ding{55} / \checkmark
&$90.9_{\pm0.8}$ & $92.2_{\pm 1.7}$
&& - & -
\\

CLIPREC (Gap Reg 1000) &
\ding{55} / \checkmark
&$91.6_{\pm0.8}$ & $93.9_{\pm1.7}$
&& - & -
\\
CLIPREC No ES (Gap Reg 1) &
\ding{55} / \checkmark
& $90.2_{\pm2.0}$& $91.0_{\pm1.5}$
&& - & -
\\
CLIPREC No ES (Gap Reg 10) &
\ding{55} / \checkmark
&$91.3_{\pm1.2}$ & $92.8_{\pm1.4}$
&& - & -
\\

CLIPREC No ES (Gap Reg 100) &
\ding{55} / \checkmark
&$90.5_{\pm0.7}$ & $91.7_{\pm1.2}$
&& - & -
\\

CLIPREC No ES (Gap Reg 1000) &
\ding{55} / \checkmark
&$90.3_{\pm0.3}$ & $92.5_{\pm1.3}$
&& - & -
\\
\\[1mm]\hline

(Analytic 1000, Train Aug 1, Train Ratio 0.8, pe None) & 
\ding{55} / \checkmark
&$\mathbf{92.6}_{\pm0.3}$ & $94.7_{\pm0.4}$
&& $\mathbf{84.7}_{\pm0.4}$ & $87.9_{\pm1.4}$
\\
\\[1mm]\hline
(Analytic 1000, Train Aug 0, CLIP Normalize) & 
\ding{55} / \checkmark
&$91.5_{\pm0.5}$ & $92.3_{\pm0.1}$
&& &
\\
(Analytic 1000, Train Aug 0.5, CLIP Normalize) & 
\ding{55} / \checkmark
&$91.8_{\pm0.5}$ & $93.2_{\pm0.7}$
&& &
\\

(Analytic 1000, Train Aug 1, CLIP Normalize) & 
\ding{55} / \checkmark
& $92.5_{\pm0.5}$ & $93.9_{\pm0.9}$
&& $84.2_{\pm0.4}$& $87.8_{\pm1.4}$
\\[1mm]\hline

(Analytic 1000, Train Ratio 1, CLIP Normalize, Orig Proj) & 
\ding{55} / \checkmark
& $92.3_{\pm0.7}$ & $93.5_{\pm1.2}$
&& $84.5_{\pm0.5}$ & $87.8_{\pm1.2}$
\\

(Analytic 1000, Train Ratio 1, CLIP Normalize, Full Proj) & 
\ding{55} / \checkmark
& $92.2_{\pm0.4}$ & $95.0_{\pm0.5}$
&& $83.6_{\pm1.1}$ & $88.7_{\pm0.9}$
\\[1mm]\hline

% (Analytic 1000, Train Ratio 1, CLIP Normalize, Reverse Proj) & 
% \ding{55} / \checkmark
% & $91.6_{\pm0.5}$ & $95.6_{\pm0.4}$
% \\[1mm]\hline

(Analytic 1000, Train Aug 1, Train Ratio 1, pe None, Full Proj) &
\ding{55} / \checkmark
&$92.1_{\pm0.3}$ & $95.8_{\pm0.5}$
&&$84.0_{\pm1.6}$ & $88.1_{\pm1.5}$
\\

(Analytic 1000, Train Aug 1, Train Ratio 1, pe None, Orig Proj) &
\ding{55} / \checkmark
&$92.5_{\pm0.5}$ & $94.5_{\pm0.6}$
&&$83.9_{\pm1.2}$ & $88.7_{\pm2.1}$
\\

(Analytic 1000,Train Aug/Ratio 1, None, Orig Proj, add gap anchor) &
\ding{55} / \checkmark
& &
&&$84.5_{\pm0.9}$ & $88.8_{\pm1.0}$

\end{tabular}

==> contents/Supp_spu_filter.tex <==
As stated in Section \ref{sec:filter}, we also try filtering $\mathcal{T}^a$ by comparing the averaged logits given by $h_\phi$ when the $t_j^a$ is present or absent.
That is, we compare $\mathbb{E}_i[\mathbb{P}(h_\phi(\Pi(\bm z^{\text{CLIP}}_{P_1(t^y_i)})) = y)]$ and $\mathbb{E}_i[\mathbb{P}(h_\phi(\Pi(\frac{\bm z^{\text{CLIP}}_{P_1(t^y_i)} + \bm z^{\text{CLIP}}_{P_1(t^a_j)}}{2})) = y)]$ for each $t^a_j$ where $t^y_i \in \mathcal{T}^y_{\text{filter}}$.
To measure the significance of the difference in means, we adopt the paired t-test.
Since the statistical test is performed on all $t^a_j \in \mathcal{T}^a_{\text{filter}}$, we need to correct the p-value of each $t^a_j$ to control the False Discovery Rate (FDR).
Therefore, we perform the Benjamini-Hochberg \cite{FDR} procedure to correct the p-values to control the FDR to be less than 0.05.
Based on this procedure, we can effectively filter $t_j^a$ which significantly affects the prediction of $h_\phi$ without introducing an additional hyperparameter.

The experimental result with the t-test based filtering is shown in the last row of Table \ref{tab:t_test}.
The effect of the t-test filter seems to be marginal.
We conjecture that the semantic filter is sufficient for $\mathcal{T}^a$.
% filtering words which affects the prediction of $h_\phi$ significantly.
To validate this conjecture, we replace the semantic filter for $\mathcal{T}^a$ with the t-test based filter and the results are shown in the second row of the Table \ref{tab:t_test}.
Indeed, the semantic filter and the t-test based filter seem to have an equivalent effect on the performance.
Hence, we use the semantic filter instead of the t-test based filter in our method because of its simplicity.

% We compare the mean logit when the text contains words about the spurious attributes and when it does not.
% That is, we compare $\mathbb{E} \mathbb{P}[\hat{y}| Pz^{\text{CLIP}}_{\text{text}_y}]$ and $\mathbb{E} \mathbb{P}[\hat{y}|P\frac{z^{\text{CLIP}}_{\text{text}_{y_i}} + z^{\text{CLIP}}_{\text{text}_{a}}}{2}]$, with expectation with respect to filtered class name synonyms.
% We evaluate the significance of the difference of mean using the paired t-test.
% Furthermore, as we perform the statistical test for every word generated for \textit{spurious attributes names}, correction of the p-value is needed to control the false discovery rate (FDR).
% Therefore, we perform the Benjamini-Hochberg procedure to correct the p-value to control the FDR to be less than 0.05.
% Based on this procedure, we can effectively filter the words that significantly affect the prediction of the trained linear classifier without introducing an additional hyperparameter.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

